PassGPT: Password Modeling and (Guided) Generation with Large Language Models

Large language models (LLMs) successfully model natural language from vast amounts of text without the need for explicit supervision. In this paper, we investigate the efficacy of LLMs in modeling passwords. We present PassGPT, a LLM trained on password leaks for password generation. PassGPT outperforms existing methods based on generative adversarial networks (GAN) by guessing twice as many previously unseen passwords. Furthermore, we introduce the concept of guided password generation, where we leverage PassGPT sampling procedure to generate passwords matching arbitrary constraints, a feat lacking in current GAN-based strategies. Lastly, we conduct an in-depth analysis of the entropy and probability distribution that PassGPT defines over passwords and discuss their use in enhancing existing password strength estimators.

==> sections/00-requirements.tex <==
\briland{Notes Feb. 4th. 2023}
\begin{itemize}
    \item Title of the paper needs revised, a couple of alternatives would be ideal.
    \item Keywords for the title: Large Language Models, Transformers, Password Guessing, Password Strength Estimation
    \item Experimental evaluation needs reordering and detailed explanation. Reordering: Password Guessing, Conditional Password Guessing, Password Strength Estimation, Insights
    \item Conform the use of PassGPT, PassVQT, PassBERT. We need to explicitly state (and illustrate) the differences between these architectures.
    \item We need a Threat Model section where we position ourselves in the \emph{offline} password guessing setting. Furthermore, we can explain the need to understand and estimate the password strength.
\end{itemize}

==> sections/06-related-work.tex <==
\section{Related Work}
\label{sec:related-work}

% \bh{Adding a list of related work to consider here:}

% \begin{enumerate}
%     \item Pasquini et al. SP'21~\cite{pasquini2021improving}
%     \item Pasquini et al. Usenix Security'21~\cite{pasquini2021reducing}
%     \item Pasquini et al. ESORICS'20~\cite{pasquini2020interpretable}
%     \item Hitaj et al. ACNS'19~\cite{hitaj2019passgan}
%     \item Pagnotta et al. DSN'22~\cite{pagnotta2022passflow}
%     \item Ciaramella et al. 2006~\cite{ciaramella2006neural}
%     \item Castelluccia et al. NDSS'12~\cite{castelluccia2012adaptive}
%     \item Dell'Amico et al. INFOCOM'10~\cite{dell2010password}
%     \item Melicher et al. Usenix Security'16~\cite{melicher2016fast}
%     \item Liu et al. SP'19~\cite{liu2019reasoning}
%     \item Blocki et al. SP'23~\cite{blocki2021towards}
%     \item Xu et al. CCS'21~\cite{xu2021chunk}
%     \item Sahin et al. CCS'21~\cite{sahin2021don}
%     \item Tan et al. CCS'20~\cite{tan2020practical}
%     \item Weir et al. SP'09~\cite{weir2009password}
%     \item Pal et al. SP'19~\cite{pal2019beyond}
%      \item Murmu et al. \cite{murmu2022passmon}
% \end{enumerate}

\subsection{Password Guessing}

\tobriland{maybe include here non-DL stuff? In any case, feel free to rearrange stuff how you feel works best for this venue :)}

\subsection{Password Strength Estimation}

I used this library which looks kind of SOTA: \url{https://dropbox.tech/security/zxcvbn-realistic-password-strength-estimation}. It is recommended in this study \cite{carnavalet2015large}

==> sections/06-remarks.tex <==
\section{Discussion}
\label{sec:remarks}

---- new added by Fernando Maybe move to some place else -----


==> sections/08-acknowledgments.tex <==
% %-------------------------------------------------------------------------------
% \section*{Acknowledgments}
% %-------------------------------------------------------------------------------

% The USENIX latex style is old and very tired, which is why
% there's no \textbackslash{}acks command for you to use when
% acknowledging. Sorry.

%-------------------------------------------------------------------------------
\section*{Availability}
%-------------------------------------------------------------------------------

The code to reproduce all the results presented in this paper is available at \texttt{hidden for submission}. Datasets can be downloaded from the respective cited sources. All code scripts are manually seeded to ensure reproducibility by third parties.

%\briland{We can use~\url{https://anonymous.4open.science/} to place a link to an anonymized version of the repository. Let's aim for a completed draft of the paper and then focus on that!}

%\jrr{I think I will not have time to prepare this before submission. If I do, I will include it here}

==> sections/09-threat-model.tex <==



